Elasticy: A Runtime-Reconfigurable Architecture for Dynamic Streams

Reconfigurable Dataflow Accelerators (RDAs) have demonstrated high performance and energy efficiency for dense, regular tensor applications. However, conventional RDAs with static configurations show dramatically reduced performance and efficiency on irregular tensor workloads with data-dependent, non-uniform, dynamic tensor shapes. We propose Elasticy, a dynamically reconfigurable dataflow accelerator that employs streaming and tile abstractions to minimize the overhead of dynamic support. By encoding dynamic shapes into streams using rank-variable expressions, Elasticy exploits data-dependent tensor shape dynamism to minimize off-chip data traffic and wasted compute cycles. Elasticy employs stream-embedded reconfiguration information to trigger fine-grained runtime scheduling decisions. Elasticy also introduces a novel distributed linked streaming memory (DLSM) that more effectively uses on-chip memory to minimize off-chip data traffic and support dynamically sized tensors. Both reconfiguration and shape dynamism incur minimal overhead in Elasticy: reconfiguration occurs infrequently at the granularity of a stream of tiles, while rank-variable expressions enable lightweight handling of dynamic dimensions. On a Llama 3-8B decode layer, Elasticy achieves 92.6% of its roofline performance, compared to 69.7% on an H100. On evaluated GEMMs, the DLSM reduces total off-chip traffic by up to 61.4% relative to the best evaluated cache configuration, with no additional burden of programmer-managed memory. Elasticy's distributed runtime scheduler overlaps dependent kernels, speeding up kernel pairs by up to 1.42x. Programs can also run in both space and time: each phase of a layer's graph is pipelined spatially, while phases fold onto the same fabric over time. Compared to a traditional spatial accelerator, Elasticy achieves a 6.34x-31.67x improved area delay product on full layers.

==> figs/eval_plot_style.tex <==
% Shared pgfplots look (kernel-over-kernel traffic bar chart). Use with \input{figs/eval_plot_style}.
% Bar colors use Okabe–Ito (figs/okabe_ito.tex, loaded from main.tex).
\pgfplotsset{
    eval traffic plot/.style={
        grid=major,
        grid style={dotted, gray!50},
        tick label style={font=\small},
        label style={font=\small},
        title style={font=\small\bfseries},
    },
    eval bar colors A/.style={fill=oiBlue!58, draw=oiBlue!88!black},
    eval bar colors B/.style={fill=oiVermillion!52, draw=oiVermillion!88!black},
    eval ref line y/.style={
        extra y ticks={#1},
        extra y tick style={grid=major, grid style={ink!50, thick, dashed}},
        extra y tick labels={},
    },
}

